Semantic Predicate Types and Approximation for Class-based Object Oriented Programming

We apply the principles of the intersection type discipline to the study of class-based object oriented programs and; our work follows from a similar approach (in the context of Abadi and Cardelli's Varsigma-object calculus) taken by van Bakel and de'Liguoro. We define an extension of Featherweight Java, FJc and present a predicate system which we show to be sound and expressive. We also show that our system provides a semantic underpinning for the object oriented paradigm by generalising the concept of approximant from the Lambda Calculus and demonstrating an approximation result: all expressions to which we can assign a predicate have an approximant that satisfies the same predicate. Crucial to this result is the notion of predicate language, which associates a family of predicates with a class.

==> commands.tex <==
\makeatletter

\def\myscriptfont{\fontsize{\@vipt}{8pt}\selectfont}

\def \psk {\hspace*{1pt}}

\newcommand{\Comment}[1]{}

\def \longharpoon#1{\psset{unit=1pt,linewidth=0.35pt}%
\psline{cc-cc}(0,1)(#1,1)%
\hspace*{#1}%
\pscurve{cc-cc}(0,1)(-1.1,1.5)(-1.75,2.25)\hspace*{.1#1}}

\renewcommand{\Vec}[2][]{%
\setbox154=\hbox{$#2$}
\setbox155=\hbox{${#2}_{#1}$}
\leavevmode
\raise\ht154\hbox{\longharpoon{\wd154}}%
\kern-1.1\wd154% put argument and move left
\box155}

%\newcommand{\typeCompatible}[1][\mvSmallExecutionContext]{\ensuremath{{\lhd \kern-0.15em\rhd}_{#1}}\xspace}

\def\arrow{\,{\rightarrow}\,}

\def\rulename#1{\mbox{{\small \sc #1}}}
\def\myvarmathbb#1{\mbox{\footnotesize $\varmathbb{#1}$}}

\def \n {\overline{n}}
\def \ele {\,{\in}\,}
\def \nele {\,{\notin}\,}

%\newcommand{\assumption}{\textrm{ass.}}
%\newcommand{\theorem}{\textrm{Thm.}}
%\newcommand{\lemma}{\textrm{Lem.}}
%\newcommand{\corollary}{\textrm{\Cor.}}

\newcommand{\CSharp}{C\#\xspace}
\newcommand{\LightweightJava}{\textsc{lj}\xspace}
\newcommand{\theLanguage}{\textit{p}\textsc{fj}\xspace}
\newcommand{\FeatherweightJava}{\textsc{fj}\xspace}
\newcommand{\GenericJava}{\textsc{gj}\xspace}
\newcommand{\MiddleweightJava}{\textsc{mj}\xspace}
\newcommand{\Varsigma}{\ensuremath{\varsigmaup}\xspace}
\newcommand{\VarsigmaCalculus}{\ensuremath{\varsigmaup}-calculus\xspace}
\newcommand{\LC}{\ensuremath{\lambda}-calculus\xspace}

\newcommand{\Undefined}{\textrm{Undefined}}

\newcommand{\mvPredicateType}[1][\phi]{\ensuremath{#1}\xspace}
\newcommand{\mvMemberPred}[1][\tau]{\ensuremath{#1}\xspace}
\newcommand{\mvObjectPredicate}{\ensuremath{\sigma}\xspace}
\newcommand{\mvUnitPredicate}{\ensuremath{\upsilon}\xspace}
\newcommand{\mvNormalPredicate}{\ensuremath{\nu}\xspace}
%\newcommand{\NullPred}{\ensuremath{N}\xspace}
\newcommand{\NullPred}{\ensuremath{\mathfrak{N}}\xspace}

\newcommand{\mvFieldType}{\ensuremath{\varphi}\xspace}
\newcommand{\mvMethodType}{\ensuremath{\mu}\xspace}
\newcommand{\mvExprType}[1][\mvClass]{\ensuremath{\mvClass[#1]}\xspace}

\newcommand{\setFieldType}{\ensuremath{\myvarmathbb{TYPE}_{\scriptsize\textsf{f}}}\xspace}
\newcommand{\setMethodType}{\ensuremath{\myvarmathbb{TYPE}_{\scriptsize\textsf{m}}}\xspace}
\newcommand{\setExprType}{\ensuremath{\myvarmathbb{TYPE}_{\scriptsize\textsf{e}}}\xspace}
\newcommand{\setClassType}{\ensuremath{\myvarmathbb{TYPE}_{\scriptsize\textsf{C}}}\xspace}
\newcommand{\setPredicates}{\ensuremath{\myvarmathbb{PRED}}\xspace}

\newcommand{\fieldId}[1][f]{\keyword{#1}}
\newcommand{\methodName}[1][m]{\keyword{#1}}
\newcommand{\className}[1][C]{\keyword{#1}}
\newcommand{\variable}[1][x]{\keyword{#1}}

\newcommand{\emptyPredicate}{\mkPredicate{\,}}%{{\emptySequence}}
\newcommand{\universalPredicate}{\ensuremath{\top}\xspace}

\newcommand{\grammaticalOr}{\ensuremath{\ \arrowvert\ }}

\newcommand{\ObjectClass}{\keyword{Object}\xspace}

\def \mvClassaux[#1]{\mbox{\rm{#1}}\xspace}
\def \mvClass{C}%\@ifnextchar[{\mvClassaux}{\ensuremath{\rm{C}}\xspace}}
\def \mvClass{\@ifnextchar[{\mvClassaux}{\mbox{\rm{C}}\xspace}}

\newcommand{\mvField}{\mbox{${f}$}\xspace}
\newcommand{\mvMethod}{\ensuremath{m}\xspace}
\newcommand{\mvLabel}{\ensuremath{\ell}\xspace}

\newcommand{\mvTermVar}[1][x]{\ensuremath{#1}\xspace}

\newcommand{\mvClassTable}[1][\mvProgram]{\ensuremath{\Delta_{#1}}\xspace}
\newcommand{\mvMethodTable}[1][\mvProgram]{\ensuremath{\Delta_{#1}^{\rm{m}}}\xspace}
\newcommand{\mvFieldTable}[1][\mvProgram]{\ensuremath{\Delta_{#1}^{\rm{f}}}\xspace}

%\newcommand{\classTable}{\ensuremath{\Delta}\xspace}
\newcommand{\classTable}{{\mbox{\small ${\cal C\kern-2pt T}$}}}

\newcommand{\methodTable}{{\mbox{\small ${\cal M\kern-1pt T}$}}\xspace}
\newcommand{\fieldTable}{{\small \mbox{${\cal F\kern-1pt T}$}}\xspace}

\newcommand{\mvTypeEnvironment}{\ensuremath{\Gamma}\xspace}
\newcommand{\mvPredicateEnvironment}{\ensuremath{\Pi}\xspace}

\newcommand{\mvSmallExecutionContext}{\mbox{\myscriptfont ${\cal E\kern-.2em C}$}}
\newcommand{\mvExecutionContext}{\mbox{{\small ${\cal E\kern-2pt C}$}}%{\chiup}
\xspace}
\newcommand{\mvProgram}{\ensuremath{%\small \rm{P}
P}\xspace}
\newcommand{\mvClassDef}{\mbox{{\small $\mathsf{cd}$}}\xspace}
\newcommand{\mvFieldDef}{\mbox{{\small $\mathsf{fd}$}}\xspace}
\newcommand{\mvMethodDef}{\mbox{{\small $\mathsf{md}$}}\xspace}
\newcommand{\mvExpression}{\mbox{{\small $\mathsf{e}$}}\xspace}
\newcommand{\mvClosedExpression}{\ensuremath{\mathfrak{e}}\xspace}
\newcommand{\mvObject}{\mbox{{\small $\mathsf{o}$}}\xspace}

\newcommand{\subscrPredType}{\kern-3pt\mbox{\textsc{\scriptsize pt}}}
%\newcommand{\subscrPredicate}{\kern-3pt\mbox{\scriptsize{$\rho$}}}

\newcommand{\typeAssRelationSym}{\vdash\xspace}
\newcommand{\typeAss}[4][\mvSmallExecutionContext]{\ensuremath{#2 \typeAssRelationSym #3{:}#4}\xspace}
\newcommand{\predAssRelationSym}{\vdash\xspace}
\newcommand{\predicateAss}[5][\mvSmallExecutionContext]{\ensuremath{#2 \predAssRelationSym #3{:}#4\,{:}\,#5}\xspace}

\newcommand{\nTypeAssRelationSym}{\nvdash^{\kern-0.35em\raise-0.05em\hbox{\scriptsize \sc t}}}
\newcommand{\nTypeAss}[4][\mvExecutionContext]{\ensuremath{#2 \nTypeAssRelationSym_{\kern-0.3em\raise 0.2em\hbox{\scriptsize{$#1$}}} #3\,{:}\,#4}\xspace}

\newcommand{\plainMemberSequence}[3][n]{\ensuremath{\Vec[#1]{#2\,{:}\,#3}}\xspace}
\newcommand{\memberSequence}[3][n]{\ensuremath{\Vec[#1]{#2\,{:}\,#3}}\xspace}
\newcommand{\superscriptedMemberSeq}[4][n]{\ensuremath{\Vec[#1]{#2^{#4}\,{:}\, #3^{#4}}}\xspace}

\newcommand{\mkPredicateAux}[1]{\ensuremath{\langle #1 \rangle}\xspace}
\def \mkPredicateBr<#1>{\ensuremath{\langle #1 \rangle}\xspace}
\def \mkPredicate{\@ifnextchar<{\mkPredicateBr}{\mkPredicateAux}}

\newcommand{\mkUPred}[2]{\mkPredicate{#1 \,{:}\, #2}}

\newcommand{\predicateMemberSeq}[1][n]{\memberSequence[#1]{\mvLabel}{\mvMemberPred}}
\newcommand{\superscriptedPredicateMemberSeq}[2][n]{\superscriptedMemberSeq[#1]{\mvLabel}{\mvMemberPred}{#2}}

\newcommand{\PredicateNoStar}[1][n]{\mkPredicate{\predicateMemberSeq[#1]}\xspace}
\newcommand{\StarredPredicate}[1][n]{\mkPredicate {\superscriptedPredicateMemberSeq[#1]{\prime}}\xspace}
\def \Predicate{\@ifstar{\StarredPredicate}{\PredicateNoStar}}

\newcommand{\selfTypeOf}{\ensuremath{ :: }}

\newcommand{\subclassLookup}{\ensuremath{\prec}\xspace}
\newcommand{\subclassOf}[1][\mvExecutionContext]{\ensuremath{\prec_{#1}}\xspace}

\newcommand{\subtypeLookup}{\ensuremath{<\colon}\xspace}
\newcommand{\subtypeOf}[1][]{\mathrel{<:}}%{\ensuremath{\ {<:}_{#1}\ }}
\newcommand{\typeCompatible}[1][\mvSmallExecutionContext]{\ensuremath{\ {<:>}_{#1}\ }}

\newcommand{\subEnvironmentOf}[1][\mvProgram]{\subtypeOf[#1]}

\newcommand{\subpredicateOf}{\ensuremath{\trianglelefteqslant}\xspace}
\newcommand{\predicateEquivalentTo}{\ensuremath{\sim}\xspace}

%\newcommand{\typeCompatible}[1][\mvSmallExecutionContext]{\ensuremath{\bowtie_{#1}}\xspace}

\newfont{\codefont}{pcrr at 9pt}
\newcommand{\code}[1]{\mbox{\codefont #1}\xspace}
\newcommand{\keyword}[1]{\mbox{\codefont #1}\xspace}

\newcommand{\spacedldots}{\ensuremath{\ \ldots\ }}
\newcommand{\spacedAmpersand}{\ensuremath{\ \&\ }}

\newcommand{\mvFieldMap}{\ensuremath{\mathbb{F}}\xspace}

\newcommand{\setProgram}{\ensuremath{\myvarmathbb{PROGRAM}}\xspace}
\newcommand{\setExecutionContext}{\ensuremath{\myvarmathbb{CONTEXT}}\xspace}
\newcommand{\setExpression}{\ensuremath{\myvarmathbb{EXPR}}\xspace}

\newcommand{\setFieldId}{\ensuremath{\myvarmathbb{FIELD}\textrm{-}\myvarmathbb{ID}}\xspace}
\newcommand{\setMethodName}{\ensuremath{\myvarmathbb{METHOD}\textrm{-}\myvarmathbb{NAME}}\xspace}
\newcommand{\setClassName}{\ensuremath{\myvarmathbb{CLASS}\textrm{-}\myvarmathbb{NAME}}\xspace}
\newcommand{\setTermVar}{\ensuremath{\myvarmathbb{VARIABLE}}\xspace}
\newcommand{\setObject}{\ensuremath{\myvarmathbb{OBJECT}}\xspace}

\newcommand{\QuantificationConditions}[1]{\ensuremath{\Quant[#1]}}

\newcommand{\subscriptedSeq}[2][n]{\ensuremath{\underline{#2}_{#1}}\xspace}
\newcommand{\unsubscriptedSeq}[1]{\ensuremath{\underline{#1}}\xspace}
\def \sequence{\@ifstar{\unsubscriptedSeq}{\subscriptedSeq}}

\newcommand{\bottom}{\ensuremath{\bot}\xspace}

\newcommand{\oneStepReducesTo}{\oneStepReductionRelation}
\newcommand{\oneStepReductionRelation}[1][]{\ensuremath{\rightarrow_{\kern-1pt#1}}\xspace}
\newcommand{\oneStepReduction}[3][]{\ensuremath{#2 \oneStepReductionRelation[#1] #3}\xspace}
\newcommand{\reductionRelation}[1][]{\ensuremath{\rightarrow^{\ast}}\xspace}
\newcommand{\reducesTo}[3][\mvSmallExecutionContext]{\ensuremath{#2 \reductionRelation[#1] #3}\xspace}

\newcommand{\reduces}{\rightarrow_{\mvSmallExecutionContext}}

\newcommand{\betaReducesTo}{\ensuremath{\rightarrow_{\beta}}}

\newcommand{\classnameLookup}{\ensuremath{\textsc{cn}}\xspace}
\newcommand{\methodNameLookup}{\ensuremath{\textsc{mn}}\xspace}
\newcommand{\fieldNameLookup}{\ensuremath{\textsc{fn}}\xspace}

\def\SuperCl{\ensuremath{\textsl{SuperCl}}\xspace}
\def\SuperClf(#1,#2){\SuperCl\,({#1},#2)}%{\SuperCl_{#1}\,(#2)}
\def\superclassLookup{\@ifnextchar({\SuperClf}{\SuperCl}}

\newcommand{\fieldListLookup}{\mbox{{\small $\cal F$}}\xspace}
\newcommand{\methodListLookup}{\mbox{{\small $\cal M$}}\xspace}
\newcommand{\methodLookup}{\mbox{{\small $\cal M$\kern-1pt\textsl{b}}}\xspace}
\newcommand{\variableLookup}{\mbox{{\small $\cal V$\kern-1pt\textsl{ars}}}\xspace}

\def \wellFormed{\@ifstar{\wellFormedNoDiamond}{\diamondWellFormed}}
\newcommand{\diamondWellFormed}[2][]{\ensuremath{#1 \vdash #2 \diamond}\xspace}
\newcommand{\wellFormedNoDiamond}[2][]{\ensuremath{#1 \vdash #2}\xspace}

\newcommand{\environmentWellFormed}[2][\mvExecutionContext]{\ensuremath{#1 \vdash #2}}

\newcommand{\typeValid}[2][\mvSmallExecutionContext]{\ensuremath{\vdash_{\kern-3pt #1} #2}}
\newcommand{\contextTypeConsistent}[1][\mvSmallExecutionContext]{\ensuremath{\typeAssRelationSym_{\kern-0.3em%\raise 0.2em
\hbox{\scriptsize {$#1$}}}\kern-0.2em\hbox{$\diamond$}}\xspace}

\newcommand{\emptySequence}{\ensuremath{\epsilonup}\xspace}

\newcommand{\acyclic}[1]{\ensuremath{\vdash #1\ \textbf{acyclic}}\xspace}
\newcommand{\extends}{\ensuremath{\prec}\xspace}

\newcommand{\substitution}[1]{\ensuremath{[#1]}\xspace}

\newcommand{\RuleNoSubscript}[1]{$\textsc{#1}$}
\newcommand{\RuleSubscript}[2]{\ensuremath{\textsc{#1}_{#2}}}
\def \RuleBr (#1){(\textsc{#1})}

\def \Rule{\@ifnextchar({\RuleBr}{\@ifstar{\RuleSubscript}{\RuleNoSubscript}}}

% \newcommand{\OneTo}[1]{\sequence*{#1}}

\newcommand{\toTypeEnvironment}[1]{#1}

\newcommand{\NewObject}[2][\mvClass]{\setbox167=\hbox{$#2$}%
\ifdim\wd167>10pt
\ensuremath{\keyword{new}\ \mvClass[#1](\psk#2\psk)}%
\else 
\ifdim\wd167>1pt
\ensuremath{\keyword{new}\ \mvClass[#1](#2)}%
\else 
\ensuremath{\keyword{new}\ \mvClass[#1](\,)}%
\fi
\fi
}

\newcommand{\PredComp}[3][\mvSmallExecutionContext]{\ensuremath{[#2]_{#1}^{\mbox{\myscriptfont ${#3}$}}}\xspace}

\newcommand{\functionSymbol}{\ensuremath{F}\xspace}
\newcommand{\functionArg}{\ensuremath{\rm{arg}}\xspace}
\newcommand{\IsDefined}{\ensuremath{\kern-0.1em\hbox{$\downarrow$}}}
\newcommand{\NotDefined}{\ensuremath{\kern-0.1em\hbox{$\uparrow$}}}

\newcommand{\Null}[1][\mvClass]{\keyword{null}}

\newcommand{\predJoinRelationSym}{\ensuremath{\sqcup}\xspace}
\newcommand{\bigPredJoinRelationSym}{\ensuremath{%\bigsqcup
\sqcup}\xspace}
\newcommand{\predicateJoin}[2]{\ensuremath{#1 \predJoinRelationSym #2}\xspace}%{\ensuremath{#1 {\sqcup \kern-0.5em\raise 0.1em\hbox to 0pt{\scriptsize P}} \kern 0.5em\hbox{\ensuremath{#2}}}\xspace}
\newcommand{\bigPredicateJoin}[2][]{\ensuremath{\mbox{} \bigPredJoinRelationSym_{#1} #2}}

\newcommand{\environmentJoin}[2]{\predicateJoin{#1}{#2}}
\newcommand{\bigEnvironmentJoin}[2][]{\bigPredicateJoin[#1]{#2}}

\newcommand{\exprJoin}[2]{\predicateJoin{#1}{#2}}
\newcommand{\bigExprJoin}[2][]{\bigPredicateJoin[#1]{#2}}

\newcommand{\typeEnvVars}{\ensuremath{\myvarmathbb{VARS}_{\rm{\scriptsize ENV}}^{\mathsc{\scriptsize t}}}\xspace}
\def\tEVaux(#1){#1}
\def\typeEnvVars{\@ifnextchar({\tEVaux}{\tEVaux()}}

\newcommand{\predEnvVars}{\ensuremath{\myvarmathbb{VARS}_{\rm{\scriptsize ENV}}^{\mathsc{\scriptsize p}}}\xspace}
\def\pEVaux(#1){#1}
\def\predEnvVars{\@ifnextchar({\pEVaux}{\pEVaux()}}

\newcommand{\mySet}[2]{\ensuremath{\{\,#1 \mid #2\,\}}\xspace}

\def\oldSet#1{\ensuremath{\{\,{#1}\,\}}\xspace}
\def\mySet#1|#2 {\ensuremath{\{\,#1 \mid #2\,\}}\xspace}
%\def\Set#1|#2{\ensuremath{\{\,#1 \mid #2\,\}}\xspace}
\def\Set#1{\@ifnextchar|{\mySet{#1}}{\oldSet{#1}}}
\def\setConstruction#1#2 {\ensuremath{\{\,#1 \mid #2\,\}}\xspace}

\newcommand{\setRankZero}{\ensuremath{\myvarmathbb{PRED}_{\textrm{\small 0}}}\xspace}
\newcommand{\setRankOne}{\ensuremath{\myvarmathbb{PRED}_{\textrm{\small 1}}}\xspace}

\newcommand{\mvRankZeroPredicateType}{\ensuremath{\alpha}\xspace}
\newcommand{\mvRankOnePredicateType}{\ensuremath{\beta}\xspace}

\newcommand{\mvRankZeroPredicateEnvironment}{\ensuremath{{\mvPredicateEnvironment^{0}}}\xspace}
\newcommand{\mvRankOnePredicateEnvironment}{\ensuremath{{\mvPredicateEnvironment^{1}}}\xspace}

\newcommand{\mvPredicateVar}{\ensuremath{\varphi}\xspace}
\newcommand{\predicateSubstitution}[2][\mvPredicateVar]{\ensuremath{(#1 \mapsto #2)}\xspace}
\newcommand{\mvPredicateSubstitution}{\ensuremath{\mathcal{S}}\xspace}

\newcommand{\rankZeroPredicateMemberSeq}[1][n]{\memberSequence[#1]{\mvField}{\mvRankZeroPredicateType}}
\newcommand{\superscriptedRankZeroPredicateMemberSeq}[2][n]{\superscriptedMemberSeq[#1]{\mvField}{\mvRankZeroPredicateType}{#2}}

\newcommand{\rankOnePredicateMemberSeq}[1][n]{\memberSequence[#1]{\mvLabel}{\mvMemberPred}}
\newcommand{\superscriptedRankOnePredicateMemberSeq}[2][n]{\superscriptedMemberSeq[#1]{\mvLabel}{\mvMemberPred}{#2}}

\newcommand{\identitySubstitution}{\ensuremath{\textit{Id}_{\mathcal{S}}}\xspace}
\newcommand{\closingSubstitution}{\ensuremath{\mvPredicateSubstitution_{\downarrow}}\xspace}

\newcommand{\unificationFunction}[1][]{\ensuremath{\textit{unify}}\xspace}
\newcommand{\unify}[2]{\ensuremath{\unificationFunction\ #1\ #2}\xspace}
\newcommand{\unifyEnvFunction}[1][]{\ensuremath{\textit{UnifyEnv}}\xspace}
\newcommand{\unifyEnv}[2]{\ensuremath{\unifyEnvFunction\ #1\ #2}\xspace}

\newcommand{\rankZeroUnificationFunction}{\unificationFunction[0]}
\newcommand{\rankZeroUnify}[2]{\ensuremath{\rankZeroUnificationFunction \ #1\ #2}\xspace}

\newcommand{\rankOneUnificationFunction}{\unificationFunction[1]}
\newcommand{\rankOneUnify}[2]{\ensuremath{\rankOneUnificationFunction \ #1\ #2}\xspace}

\newcommand{\rankZeroUnifyEnvFunction}{\ensuremath{\textit{UnifyEnv}_{0}}\xspace}
\newcommand{\rankZeroUnifyEnv}[2]{\ensuremath{\rankZeroUnifyEnvFunction \ #1\ #2}\xspace}

\newcommand{\rankOneUnifyEnvFunction}{\ensuremath{\textit{UnifyEnv}_{1}}\xspace}
\newcommand{\rankOneUnifyEnv}[2]{\ensuremath{\rankOneUnifyEnvFunction \ #1\ #2}\xspace}

\newcommand{\predicateMatchFunction}{\ensuremath{\textit{match}}\xspace}
\newcommand{\predicateMatch}[2]{\ensuremath{\predicateMatchFunction\ #1\ #2}\xspace}

\newcommand{\predicateOverrideFunction}{\ensuremath{\textit{override}}\xspace}
\newcommand{\predicateOverride}[3][\mvField]{\ensuremath{\predicateOverrideFunction\ #1\ #2\ #3}\xspace}

\newcommand{\True}{\textsc{true}\xspace}
\newcommand{\False}{\textsc{false}\xspace}

\newcommand{\rankZeroPredicateInferenceFunction}{\ensuremath{\textit{Inf}_{0}}\xspace}
\newcommand{\rankZeroPredicateInf}[3]{\ensuremath{\rankZeroPredicateInferenceFunction\ (#1, #2, #3)}\xspace}

\newcommand{\rankOnePredicateInferenceFunction}{\ensuremath{\textit{Inf}_{1}}\xspace}
\newcommand{\rankOnePredicateInf}[3]{\ensuremath{\rankOnePredicateInferenceFunction\ (#1, #2, #3)}\xspace}

\newcommand{\rankZeroOpenPredicateInferenceFunction}{\ensuremath{\mathcal{R}_{0}}\xspace}
\newcommand{\rankZeroOpenPredicateInf}[3]{\ensuremath{\rankZeroOpenPredicateInferenceFunction\ (#1, #2, #3)}\xspace}

\newcommand{\rankOneOpenPredicateInferenceFunction}{\ensuremath{\mathcal{R}_{1}}\xspace}
\newcommand{\rankOneOpenPredicateInf}[3]{\ensuremath{\rankOneOpenPredicateInferenceFunction\ (#1, #2, #3)}\xspace}

\newcommand{\flattenPredicate}[1]{\ensuremath{\lfloor #1 \rfloor}\xspace}

\newcommand{\predicateCombinationSymbol}{\ensuremath{+}\xspace}
\newcommand{\combinePredicates}[2]{\ensuremath{#1 \predicateCombinationSymbol #2}\xspace}
\newcommand{\predicateSum}[2][n]{\ensuremath{\Sigma_{\OneTo{#1}}\ #2}\xspace}
\newcommand{\combineEnv}[2]{\ensuremath{\combinePredicates{#1}{#2}}\xspace}
\newcommand{\environmentSum}[2][n]{\ensuremath{\predicateSum[#1]{#2}}\xspace}

\newcommand{\freshPredicate}[1]{\ensuremath{\textit{FreshPredicate}_{#1}}\xspace}

\newcommand{\pairSeparator}{\ensuremath{, \;}}

\newcommand{\typeInfFunction}{\ensuremath{\textit{Type}}\xspace}
\newcommand{\typeInf}[3][\mvExecutionContext]{\ensuremath{\typeInfFunction\ (#1, #2, #3)}\xspace}


\newcommand{\VarsigmaObjectFragment}{\ensuremath{\textbf{Ob}_{\textbf{\small 1}}}\xspace}
\newcommand{\VarsigmaOneTo}[1][n]{\ensuremath{1..#1}\xspace}
\newcommand{\VSObjType}[1][n]{\ensuremath{[{\mvLabel_{i}{:}B_{i}}^{\hspace{1pt} i \in \VarsigmaOneTo[#1]}]}\xspace}
\newcommand{\VSObject}[1][n]{\ensuremath{[{\mvLabel_{i}{:}\Varsigma(\mvTermVar^{A_{i}})b_{i}}^{\hspace{1pt} i \in \VarsigmaOneTo[#1]}]}\xspace}
\newcommand{\updatedBy}{\ensuremath{\ {\raise 1pt\hbox to 0pt{$\leftharpoonup$}\raise-1pt\hbox{$\leftharpoondown$}}\ }\xspace}
\newcommand{\VSObjectSubstitution}[2]{\ensuremath{\{#1 \leftarrow #2\}}\xspace}
\newcommand{\evaluatingContext}[1]{\ensuremath{\mathcal{E}[#1]}\xspace}
\newcommand{\VarsigmaObjectAssignment}[3][E]{\ensuremath{#1 \vdash_{\textsc{\scriptsize o}} #2 : #3}\xspace}
\newcommand{\VarsigmaPredicateAssignment}[4][\Gamma]{\ensuremath{#1 \vdash_{\textsc{\scriptsize p}} #2 : #3 : #4}\xspace}

\newcommand{\Derivation}{\ensuremath{\mathcal{D}}\xspace}
\newcommand{\derives}[2][\Derivation]{\ensuremath{#1 {:}{:} #2}\xspace}

\newcommand{\computabilityPredicate}[4]{\ensuremath{\mathit{Comp}(#1,#2{:}#3,#4)}\xspace}
\newcommand{\mvApprExpr}{\mbox{{\small $\mathsf{a}$}}\xspace}
\newcommand{\mvApprNF}{\mbox{{\small $\mathsf{A}$}}\xspace}
\newcommand{\mvUnambExpr}{\mbox{{\small $\mathsf{u}$}}\xspace}
\newcommand{\mvNeutralExpr}{\mbox{{\small $\mathsf{n}$}}\xspace}
%\newcommand{\directlyApproximates}{\ensuremath{~{\sqsubseteq}_{\mvSmallExecutionContext}~}}
\newcommand{\directlyApproximates}{\ensuremath{~{\sqsubseteq}~}}
%\newcommand{\approximates}{~\boxtilde_{\mvSmallExecutionContext}~}%{\sqsubset\kern.1pt\raise-4.5pt\hbox{$\sim$}}
\newcommand{\approximates}{~{\boxtilde}_{\mvSmallExecutionContext}~}
\newcommand{\approximantsOf}[1]{\ensuremath{\mathcal{A}(#1)}\xspace}
%\newcommand{\approximantsOf}[1]{\ensuremath{\mathcal{A}\hspace*{.5pt}(#1)}\xspace}
\newcommand{\approximationPredicate}[4]{\ensuremath{\mathit{Appr}\kern-1pt_{\mvSmallExecutionContext}(#1,#2{:}#3,#4)}\xspace}

\def \der #1 |- #2 : #3 { #1 \vdash #2 : #3 }
\def \Iff {\Leftrightarrow}
\def \Then {\Rightarrow}
\def \SetAppOne(#1){{\cal A}(#1)}
\def \SetApp{\@ifnextchar({\SetAppOne}{{\cal A}}}
\def \Quant[#1]{ ~ [ ~ #1 ~ ] }
\def \redbots	{\mbox	{$\rightarrow_{\beta\bottom}$}}
\def \redbot	{\ \redbots~}
\def \bredr	{{\rightarrow}_{\beta}}
\def \bred	{~{\bredr}~}
\def \dbredr	{{\rightarrow} \kern-.8em\bredr}
\def \dbred	{~\dbredr~}
\def \eqb {=_{`b}}
\def \tseqr	{{\sqsubseteq}}
\def \tseq	{~\tseqr~}
\def \And {~\&~}
\def \Lub	{\raise.75pt\hbox{$\bigsqcup$}}
% \def \join	{A\mathop{\sqcup}}

\def \sqsubset{\psset{linewidth=0.5pt}
	\psline{c-c}(1pt,0.4pt)(1pt,6pt)
	\psline{c-c}(1pt,6pt)(6.5pt,6pt)
	\psline{c-c}(1pt,0.4pt)(6.5pt,0.4pt)
}
\def \boxtilde{\sqsubset\kern.1pt\raise-4.5pt\hbox{$\sim$}}
\def \approximant {~{\boxtilde}~}
\def \Lb {`L\bottom}

\def \Set#1{\{\, #1 \,\}} 

\def\semcolour{}
\def\termcolour{}
\def\neutral{}

\def \AppNF	{{\termcolour \cal A}}
\setbox134=\hbox{\raise1\point\hbox{${\semcolour \lceil}\kern-3\point{\semcolour\lceil}$}}
\setbox135=\hbox{\raise1\point\hbox{${\semcolour \rfloor}\kern-3\point{\semcolour \rfloor}$}}
\def \semEl#1{\copy134{#1}\copy135\neutral }
\def \AECSem[#1]{\leavevmode\semEl{#1}}

\def \LJ {\LightweightJava}
\def \Expr {\mvExpression}
\def \TEnv {\mvTypeEnvironment}
\def \PEnv {\mvPredicateEnvironment}
\def \Clss	{\mvClass}
\def \Fld {\mvField}
\def \Pred {\mvPredicateType}
\def \NPred {\mvNormalPredicate}
\def \EC {\mvExecutionContext}
\def \NExpr {\mvNeutralExpr}
\def \Comp {\computabilityPredicate}
\def \OPred {\mvObjectPredicate}
\def \UPred {\mvUnitPredicate}
\def \Appr{\approximationPredicate}
\def \ApprNF{\mvApprNF}
\def \Coloneqq{\mbox{$::=$}}
\def \HNF{\mbox{$\cal H$}\xspace}
\def \NF{\mbox{$\cal N$}\xspace}
\def \HNFExpr{\mbox{{\small $\mathsf{H}$}}\xspace}
\def \NFExpr{\mbox{{\small $\mathsf{N}$}}\xspace}

\def \TAss{\typeAss}
\def \PAss{\predicateAss}
\def \PJoin {\predicateJoin}
\def \EJoin {\environmentJoin}

\def \QED{\mbox{~\large$\Box$}}
\def \ITD {\textsc{itd}}
\def \ML {\textsc{ml}}
\def \Let {\texttt{let}}

\def \inter {\mbox{\small $\cap$}}
\def \derI #1 |- #2 : #3 { #1 \vdash #2 : #3 }

\newcommand{\Lang}[1][\mvSmallExecutionContext]{\ensuremath{{\cal L}}}

\makeatother

